Exemplar Masking for Multimodal Incremental Learning

Multimodal incremental learning needs to digest the information from multiple modalities while concurrently learning new knowledge without forgetting the previously learned information. There are numerous challenges for this task, mainly including the larger storage size of multimodal data in exemplar-based methods and the computational requirement of finetuning on huge multimodal models. In this paper, we leverage the parameter-efficient tuning scheme to reduce the burden of fine-tuning and propose the exemplar masking framework to efficiently replay old knowledge. Specifically, the non-important tokens are masked based on the attention weights and the correlation across different modalities, significantly reducing the storage size of an exemplar and consequently saving more exemplars under the same memory buffer. Moreover, we design a multimodal data augmentation technique to diversify exemplars for replaying prior knowledge. In experiments, we not only evaluate our method in existing multimodal datasets but also extend the ImageNet-R dataset to a multimodal dataset as a real-world application, where captions are generated by querying multimodal large language models (e.g., InstructBLIP). Extensive experiments show that our exemplar masking framework is more efficient and robust to catastrophic forgetting under the same limited memory buffer. Code is available at https://github.com/YiLunLee/Exemplar_Masking_MCIL.

==> sec/2_cvpr_results.tex <==
\noindent\textbf{Studies of multimodal dataset generation.}
\alan{In this work, one of the evaluations of multimodal class-incremental learning is based on a newly proposed dataset (denoted as \textbf{MM-ImageNet-R}), which stemmed from the ImageNet-R \cite{hendrycks2021many} but has the carefully-designed multimodal extension (i.e., extended from only having image modality to having both text and image modalities). In addition to directly querying multimodal large language models (LLMs) to generate captions, we further explore another practical pipeline for obtaining the text data: generate rough captions via image captioning models first and then refine them with large language models (LLMs).
Specifically, given an image from ImageNet-R, we derive its text description automatically by using a state-of-the-art image captioning model, ClipCap \cite{mokady2021clipcap}. Since the initial captions (denoted as \texttt{CAPTION}) produced by ClipCap are usually not fruitful enough and do not describe the image content in a human-like manner, we hence further utilize the large language models (e.g., PaLM \cite{chowdhery2022palm} and ChatGPT \cite{openai2023chatGPT}) to refine the captions via querying LLMs with the following prompts: ``You are the imaginative storyteller. Revise the description: ``\{\texttt{CAPTION}\}". (about 100 words)".}

\alan{We summarize the quantitative results on two variants of our MM-ImageNet-R dataset (i.e., either the initial captions from ClipCap is refined by PaLM or ChatGPT) in Table~\ref{table:quantitative_palm} and \ref{table:quantitative_chat}, respectively. We draw several observations:\\
\indent 1) Compared with the results on MM-ImageNet-R dataset which captions are generated by multimodal large language models (i.e., InstructBLIP) in the main paper, the overall performance trend is similar, but the value is much lower. \\
\indent 2) . \\
}

\begin{table}[!t]
    \centering
    \caption{Average incremental accuracy on MM-ImageNet-R (texts refined by PaLM) with different numbers of incremental phases $L$=5, 10, 20. The memory size is 5 raw multimodal samples/class. \textbf{Ours} stands for our overall exemplar masking framework, while 
    \textbf{MDA} stands for multimodal data augmentation.
    }
    \label{table:quantitative_palm}
    % \scriptsize
    \resizebox{0.6\linewidth}!{
    % \tabcolsep=0.05cm
    \begin{tabular}{ccccccc}
    \hline
    \multirow{2}{*}{Methods}  &
    \multirow{2}{*}{\shortstack{\# of \\ Parameters}} &
    \multicolumn{5}{c}{
    MM-ImageNet-R (PaLM)} \\ \cline{3-7} 
    & & $L$=5 &\color{white}{d}& $L$=10 && $L$=20 \\
    \hline % baselines
    FT  & \multirow{4}{*}{112M} & 70.61 && 66.83 && 62.20 \\
    FT + CIM~\cite{luo2023cim}  & & 71.43 && 67.79 && 63.23 \\
    FT + Ours (w/o MDA)  & & 73.13 && 70.01 && 63.94 \\
    FT + Ours  & & \textbf{73.29} && \textbf{71.07} && \textbf{64.99} \\
    \hline % baselines
    SSF  & \multirow{4}{*}{206K} & 71.10 && 67.63 && 63.24 \\
    SSF + CIM~\cite{luo2023cim}  & & 71.81 && 68.45 && 65.22 \\
    SSF + Ours (w/o MDA)  & & 73.38 && 71.82 && 67.60 \\
    SSF + Ours  & & \textbf{73.97} && \textbf{72.28} && \textbf{69.04} 
    \end{tabular}
    }
\end{table}

\begin{table}[!t]
    \centering
    \caption{Average incremental accuracy on MM-ImageNet-R (texts refined by ChatGPT) with different numbers of incremental phases $L$=5, 10, 20. The memory size is 5 raw multimodal samples/class. \textbf{Ours} stands for our overall exemplar masking framework, while 
    \textbf{MDA} stands for multimodal data augmentation.
    }
    \label{table:quantitative_chat}
    % \scriptsize
    \resizebox{0.6\linewidth}!{
    % \tabcolsep=0.05cm
    \begin{tabular}{ccccccc}
    \hline
    \multirow{2}{*}{Methods}  &
    \multirow{2}{*}{\shortstack{\# of \\ Parameters}} &
    \multicolumn{5}{c}{
    MM-ImageNet-R (ChatGPT)} \\ \cline{3-7} 
    & & $L$=5 &\color{white}{dd}& $L$=10 && $L$=20 \\
    \hline % baselines
    FT  & \multirow{4}{*}{112M} & 70.42 && 66.62 && 62.21 \\
    FT + CIM~\cite{luo2023cim}  &  & 71.89 && 68.56 && 63.86 \\
    FT + Ours (w/o MDA)  & & 73.86 && 70.78 && 64.94 \\
    FT + Ours  & & \textbf{73.57} && \textbf{71.33} && \textbf{67.37} \\
    \hline % baselines
    SSF  & \multirow{4}{*}{206K} & 71.30 && 67.66 && 64.30 \\
    SSF + CIM~\cite{luo2023cim}  & & 72.30 && 69.91 && 66.66 \\
    SSF + Ours (w/o MDA)  & & 73.50 && 71.88 && 68.40 \\
    SSF + Ours  & & \textbf{73.99} && \textbf{72.24} && \textbf{69.50} 
    \end{tabular}
    }
\end{table}
